Hypocoercivity of Piecewise Deterministic Markov Process-Monte Carlo

In this work, we establish $\mathrm{L}^2$-exponential convergence for a broad class of Piecewise Deterministic Markov Processes recently proposed in the context of Markov Process Monte Carlo methods and covering in particular the Randomized Hamiltonian Monte Carlo, the Zig-Zag process and the Bouncy Particle Sampler. The kernel of the symmetric part of the generator of such processes is non-trivial, and we follow the ideas recently introduced by (Dolbeault et al., 2009, 2015) to develop a rigorous framework for hypocoercivity in a fairly general and unifying set-up, while deriving tractable estimates of the constants involved in terms of the parameters of the dynamics. As a by-product we characterize the scaling properties of these algorithms with respect to the dimension of classes of problems, therefore providing some theoretical evidence to support their practical relevance.

==> keep_proof.tex <==
  \begin{lemma} \label{lem:linkPoincare-DMSabstract}
Assume  $ \calD \Piv  \subset \calT \Piv $, $\mct \Piv$ is closable and densily defined and \Cref{as:U}-\ref{item:liminf}. Then, for any $\ff \in \domain(\mct \Piv)$ \eqref{eq:DMS_macro} holds  with
  \begin{equation}
    \label{eq:def_lambda_x}
\lambda_x = C_x/(1+C_x) \eqsp.    
\end{equation}
% In addition the condition \eqref{eq:poincare_assumption} with $\lambda_x$ given by \eqref{eq:def_lambda_x} is   equivalent \Cref{as:U}-\ref{item:liminf}. 
\end{lemma}

\begin{proof}
% Note that in the sense of symmetric operators 
% \begin{equation}
% \begin{aligned}
% 	\frac 1 {m_2} (\calT \Piv)^* (\calT \Piv) = \frac 1 {m_2} \sum_{i,j=1}^D \Piv v_i \partial_{x_i}^* v_j \partial_{x_j} \Piv = \sum_{i=1}^D \partial_{x_i}^* \partial_{x_i} = \Piv \nax^* \nax \succeq C_x \Piv,
% \end{aligned}
% \end{equation}
% and $\calA$ can be reformulated as follows
% \begin{equation}
% 	\calA = \frac 1 {m_2} \left( 1 + \nax^* \nax \right)^{-1} \Piv \nax^* v.
% \end{equation}
% Note that since $\Piv v \Piv = 0$, then $\calA = \Piv \calA (\Id-\Piv)$. By definition of $\calA$
% \begin{equation}
% \begin{aligned}
% 	\calA \calT \Piv &= \left( 1+ \frac 1 {m_2} (\calT \Piv)^* (\calT \Piv) \right)^{-1} \frac 1 {m_2} (\calT \Piv)^* \calT \Piv \\
% 	&= \left( 1 + \nax^* \nax \right)^{-1} \nax^* \nax \Piv
% \end{aligned}
% \end{equation}
% so using that from $\eqref{eq:poincare_assumption}$ $\nax^* \nax$ is self-adjoint with spectral gap $C_x$, we get by spectral calculus
% \begin{equation}
% 	\calA \calT \Piv \succeq \lambda_x \Piv.
% \end{equation}
% where $\lambda_x = \frac {C_x}{1+C_x}$.

  Note first that from the identity for any $\ff \in \domain(\mcd \Piv)$
  \[
\int\big(\calD\Piv \ff \big)^{2}{\rm d}\nu=m_{2}\normmu{\nabla_{x}\Piv \ff }^{2}
\]
and the assumed Poincar\'e inequality \eqref{eq:poincare_assumption} we have for any $\ff \in \domain((\mcd \Piv)^{*}\mcd \Piv)$,
\begin{equation}
  \label{eq:lem_proof_poincare_dms_as}
\psmu{ \ff }{m_{2}^{-1}(\calD\Piv)^{*}\calD\Piv \ff }=\normmu{m_{2}^{-1/2}\calD\Piv \ff}^{2}=\normmu{\nax\Piv \ff}^{2}\geq \Cp\normmu{\Piv \ff}^{2} \eqsp.
\end{equation}
Since $\mcd \Piv \subset \mct \Piv$ and $\mcd \Piv$ is densily defined, we get $(\mcd \Piv)^* = (\overline{\mct \Piv})^*$. This result and \eqref{eq:lem_proof_poincare_dms_as} implies that $\spec(m_{2}^{-1}(\overline{\mct\Piv})^{*} \overline{\mct\Piv})\subseteq \coint{\Cp,\infty}$
by \cite[Theorem 5.1.9]{pedersen1995analysis} and \cite[Theorem 4.3.1]{davies:1995}.

Second, note that 
\begin{equation*}
\calA \calT\Piv \ff  =\big(m_{2}I+(\calD\Piv)^{*}\calD\Piv\big)^{-1}(\calD\Piv)^{*}\calD\Piv \ff = \Phi\big(m_{2}^{-1}(\calD\Piv)^{*}\calD\Piv\big) \ff   \eqsp,
\end{equation*}
where $\Phi(z)=(1+z)^{-1}z$. From the spectral mapping theorem \cite[Theorem 2.5.1]{davies:1995} and the fact that
$\Phi\colon \coint{0,\infty}\rightarrow \ccint{0,1}$ is non-decreasing ${\spec}\big(\calA\calT\Piv\big)\subseteq \coint{\Phi(\Cp),1}$. In addition, from  the fact that $\Piv$ is a projector, we deduce $\calA \calT\Piv \ff = \Piv\Phi\big(m_{2}^{-1}(\calD\Piv)^{*}\calD\Piv\big)\Piv \ff$ and therefore, we get 
implying 
\begin{equation*}
\psmu{\Piv \ff}{\calA\calT\Piv \ff }   =\psmu{\Piv \ff}{\Piv\Phi \big(m_{2}^{-1}(\calD\Piv)^{*}\calD\Piv\big)\Piv \ff } \geq\frac{\Cp}{1+\Cp}\normmu{\Piv \ff }^{2}=\lambda_{x}\normmu{\Piv \ff}^{2} \eqsp,
\end{equation*}
which concludes the proof.


\end{proof}


==> regularization.tex <==

\subsection{Regularization procedure for the semi-group}

The Gronwall argument used to conclude the proof of Theorem~\ref{thm:hypocoercivity} is only formal since the semi-group generated by the generator $\calL$ does not let the space $\scrC$ invariant. Due to the roughness of the jump rates $(F_k^\top v)_+$, the semi-group only keeps $\rmL^\infty$ a priori. For regularization purpose we consider for any $k \in [1,K]$ and $\delta > 0$ a function $\chi_{k,\delta} \in \scrC$ such that\todo{JR:introduce CA's jump rate which ensures that the invariant measure is preserved?}
\begin{equation}
	\| \chi_{k,\delta}(x,v) - (v^\top F_k)_+ \|_\infty \le \delta.
\end{equation}
Such a function indeed exists by density of $\scrC$ in $\rmC$ for the norm $\| \cdot \|_\infty$. Define now the Markov process of generator
\begin{equation}
	\calL_\delta := \calL + \sum_{k=1}^K \left( \chi_{k,\delta}(x,v) - (v^\top F_k)_+ \right) (R_k - 1) = \calL + \calK_\delta,
\end{equation}
for any $\delta \ge 0$, then $\| \calK_\delta \| \le \delta K$ as an operator on $\Lmu$ and $\calK_\delta = \calK_\delta (1 - \Piv)$. The semi-group generated by $\calL_\delta$ lets $\scrC$ invariant \todo{JR: to be proved}, so that for any $f \in \scrC$ and $t \ge 0$, we can define $f_t^\delta = \rme^{t \calL_\delta} f \in \scrC$. Moreover
\begin{equation}
\begin{aligned}
	\frac \rmd {\rmd t} \calH[f_t^\delta] &= -\msd[f_t^\delta] + \lang \calK_\delta f_t^\delta,f_t^\delta \rang + \varepsilon \lang \calK_\delta f_t^\delta , (\calA + \calA^*) f_t^\delta \rang \\
	&\le -\msd[f_t^\delta] + \| \calK_\delta f_t^\delta \| \left( \| f_t^\delta \| + \varepsilon \left[ \| A f_t^\delta \| + \| A^* f_t^\delta \| \right] \right) \\
	&\le -\msd[f_t^\delta] + \delta K (1 + \varepsilon) \| (1-\Piv) f_t^\delta \| \left( \| \Piv f_t^\delta \| + \| (1-\Piv) f_t^\delta \| \right) \\
	&\le -\msd[f_t^\delta] + 4 K \delta \| f_t^\delta \|^2 \\
	&\le -(\Lambda(\varepsilon) - 4 K \delta) \| f_t^\delta \|^2 \\
\end{aligned}
\end{equation}
\todo{JR:a rough estimate is sufficient, this computation can be made shorter...}
For $\delta$ sufficiently small we obtain
\begin{equation}
	\left\| \rme^{t \calL_\delta} f \right\| \le C \rme^{-\nu_\delta t} \| f \|,
\end{equation}
where $\nu_\delta = \nu + \calO(\delta)$ is a perturbation of the decay rate $\nu > 0$ obtained for $\delta = 0$. In order to conclude we need a bound such as
\begin{equation}
	\left\| \rme^{t \calL} f - \rme^{t \calL_\delta} f \right\|_\infty \le \rme^{\delta t} \| f \|_\infty,
\end{equation}
for any bounded function $f$. Note that in general $\rme^{t \calL} f$ is not better than bounded a priori...


